A variational framework for modal estimation

Multivariate mode estimation arises in many statistical problems such as inverse problems, multimodal sampling, and density-based clustering, but becomes challenging in moderate to high dimensions, especially when the underlying density is not directly evaluable. We introduce GERVE (Gibbs-measure Entropy-Regularized Variational Estimation), a sample-based method for estimating multivariate modes by approximating Gibbs distributions directly from samples, without estimating or evaluating the density. GERVE uses Gaussian-mixture variational annealing and natural-gradient optimization, producing a mixture concentrated in high-density regions whose component responsibilities also provide a clustering of the observations. We prove theoretical guarantees in two regimes: as the Gibbs temperature goes to zero, the optimal variational mixture concentrates around the global modes of the population density; at fixed positive temperature, we prove existence, consistency, and asymptotic normality of empirical maximizers and propose a bootstrap procedure for uncertainty quantification. Simulations and a real-data experiment show that GERVE accurately recovers modes and produces meaningful clusters.

==> preamble.tex <==

\usepackage{url}
\usepackage{graphicx}
\usepackage{amssymb,amsmath,enumerate}
\usepackage{amsthm}
\graphicspath{{pics/}{figs/}}
\usepackage{afterpage}
\usepackage{textcomp}
\RequirePackage{amsmath} \RequirePackage{xspace}

\usepackage{empheq}
\usepackage[most]{tcolorbox}

\usepackage{svg}
\usepackage{booktabs}

% \usepackage[margin=1.2in]{geometry}
\usepackage{enumitem}
% Remove vertical space before (and inside) all itemize/enumerate lists:
\setlist[itemize,enumerate]{topsep=0pt, partopsep=0pt, parsep=0pt, itemsep=0pt}

% Theorem, prop etc...
\newcommand{\lyxaddress}[1]{
	\par {\raggedright #1
	\vspace{1.4em}
	\noindent\par}
}
\newenvironment{lyxlist}[1]
	{\begin{list}{}
		{\settowidth{\labelwidth}{#1}
		 \setlength{\leftmargin}{\labelwidth}
		 \addtolength{\leftmargin}{\labelsep}
		 \renewcommand{\makelabel}[1]{##1\hfil}}}
	{\end{list}}
\theoremstyle{plain}
\newtheorem{theorem}{{Theorem}}[section] 
\newtheorem*{theorem*}{{Theorem}}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem*{assumption*}{Assumption}
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}

\theoremstyle{remark}
\newtheorem*{notation*}{Notation}
\newtheorem*{remark*}{Remark}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% User specified LaTeX commands.
%\usepackage[T1,hyphens]{url}
%\usepackage{hyperref}
%
%\@ifundefined{showcaptionsetup}{}{%
% \PassOptionsToPackage{caption=false}{subfig}}
%\usepackage{subfig}
%\makeatother
%
%\usepackage{babel}
\providecommand{\corollaryname}{Corollary}
\providecommand{\lemmaname}{Lemma}
\providecommand{\definitionname}{Definition}
\providecommand{\notationname}{Notation}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}


% DEFINITIONS PRELIMINAIRES
\def\argmax{\mathop{\mathrm{arg\,max}}} % Mieux que \def\argmax{\arg\max}
\def\argmin{\mathop{\mathrm{arg\,min}}} % car l'indice est reparti
\def\tr{\mathop{\mathrm{Tr}}}
\RequirePackage{amsmath} \RequirePackage{xspace}
\RequirePackage{bbm}


\def\XS{\xspace}
\DeclareMathAlphabet{\mathb}{OML}{cmm}{b}{it}
\def\sbm#1{\ensuremath{\mathb{#1}}}                % Style gras italique (necessite amsmath)
%
\def\sbmm#1{\ensuremath{\boldsymbol{#1}}}          % Style gras italique (necessite amsmath)
\def\sdm#1{\ensuremath{\mathrm{#1}}}               % Style droit en math
\def\sbv#1{\ensuremath{\mathbf{#1}}}               % Style gras droit
\def\scu#1{\ensuremath{\mathcal{#1\XS}}}           % Style cursif
\def\scb#1{\ensuremath{\boldsymbol{\mathcal{#1}}}} % Style gras cursif
\def\sbl#1{\ensuremath{\mathbbm{#1}}}              % Style blackboard (necessite bbm)

% ALPHABET GRAS ITALIQUE, taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}
\def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}
\def\ellb{{\sbm{\ell}}\XS}

% ALPHABET GREC GRAS, taille adaptative

\def\alphab      {{\sbmm{\alpha}}\XS}
\def\betab       {{\sbmm{\beta}}\XS}
\def\gammab      {{\sbmm{\gamma}}\XS}
\def\Gammab    {{\sbmm{\Gamma}}\XS}
\def\deltab      {{\sbmm{\delta}}\XS}      \def\Deltab    {{\sbmm{\Delta}}\XS}
\def\epsilonb    {{\sbmm{\epsilon}}\XS}
\def\varepsilonb {{\sbmm{\varepsilon}}\XS}
\def\etab        {{\sbmm{\eta}}\XS}
\def\thetab      {{\sbmm{\theta}}\XS}      \def\Thetab    {{\sbmm{\Theta}}\XS}
\def\varthetab   {{\sbmm{\vartheta}}\XS}
\def\iotab       {{\sbmm{\iota}}\XS}
\def\kappab      {{\sbmm{\kappa}}\XS}
\def\lambdab     {{\sbmm{\lambda}}\XS}    \def\Lambdab   {{\sbmm{\Lambda}}\XS}
\def\mub         {{\sbmm{\mu}}\XS}
\def\nub         {{\sbmm{\nu}}\XS}
\def\xib         {{\sbmm{\xi}}\XS}                 \def\Xib        {{\sbmm{\Xi}}\XS}
\def\pib         {{\sbmm{\pi}}\XS}                 \def\Pib        {{\sbmm{\Pi}}\XS}
\def\varpib      {{\sbmm{\varpi}}\XS}
\def\rhob        {{\sbmm{\rho}}\XS}
\def\varrhob     {{\sbmm{\varrho}}\XS}
\def\sigmab      {{\sbmm{\sigma}}\XS}      \def\Sigmab    {{\sbmm{\Sigma}}\XS}
\def\varsigmab   {{\sbmm{\varsigma}}\XS}  \def\Varsigmab {{\sbmm{\Varsigma}}\XS}
\def\phib        {{\sbmm{\phi}}\XS}        \def\Phib       {{\sbmm{\Phi}}\XS}
\def\varphib     {{\sbmm{\varphi}}\XS}
\def\chib        {{\sbmm{\chi}}\XS}
\def\psib        {{\sbmm{\psi}}\XS}        \def\Psib       {{\sbmm{\Psi}}\XS}
\def\omegab      {{\sbmm{\omega}}\XS}      \def\Omegab    {{\sbmm{\Omega}}\XS}
\def\taub        {{\sbmm{\tau}}\XS}
\def\upsilonb    {{\sbmm{\upsilon}}\XS}   \def\Upsilonb  {{\sbmm{\Upsilon}}\XS}
\def\zetab       {{\sbmm{\zeta}}\XS}
\def\upsilonb       {{\sbmm{\upsilon}}\XS}
\def\PM{\kern0pt^{\textrm{{\scriptsize PM}}}\kern0pt}
\def\MMAP{\kern1pt^{\textrm{{\tiny MMAP}}}\kern-1pt}
\def\ML{^{\textrm{{\tiny ML}}}}
\def\dd{\,d}                            % doit etre en italique en anglais
\def\I{\,|\,}           % "sachant" bien espac\'e pour les formules


\newcommand{\w}{\omega}
\newcommand{\g}{\mathcal{G}}
\newcommand{\scalarprod}[2]{{{\bf \langle} {#1},{#2} {\bf \rangle}}}

\newcommand{\Hcondtheta}{H_{\theta\vert Y, T, S}} % loi conditionnelle
\newcommand{\HcondS}{H_{T \vert  S, Y, \theta}} % loi conditionnelle
\newcommand{\HcondT}{H_{S \vert T, Y, \theta}} % loi conditionnelle
\newcommand{\pjcomp}{p_{(Y,S,T)}} %  vraisemblance jointe complete.
\newcommand{\pjcondS}{p_{T \vert S, Y}} % loi conditionnelle
\newcommand{\pjcondT}{p_{S \vert T, Y}} % loi conditionnelle
\newcommand{\pjattach}{p_{Y \vert T, S}} % loi attache donnees
\newcommand{\pjpost}{p_{T, S \vert Y}} % loi a posteriori
\newcommand{\prior}{p_{Z}} % Loi a priori.
\newcommand{\pcomp}{p_{(Y,Z)}} %  vraisemblance complete.
\newcommand{\ppost}{p_{Z \vert Y}} % loi a posteriori
\newcommand{\pattach}{p_{Y \vert Z}} % loi a posteriori
\newcommand{\pinc}{p_{Y}} %  vraisemblance incomplete.
\newcommand{\kde}{\mathrm{kde}} % Kernel density estimate
\newcommand{\KL}{\mathrm{KL}} % Distance de Kullback-Leibler
\newcommand{\Supp}{\mathrm{Supp}} % Support loi probabilité
\newcommand{\MMD}{\mathrm{MMD}} % Maximum mean discrepancy
\newcommand{\Nv}{\mathcal{N}} %  voisinage
\newcommand{\DZe}{\mathcal{D}} % Ensemble des probabilites sur Z
\newcommand{\Ind}{\mathcal{I}} % Ensemble des probabilites independantes sur Z
\newcommand{\IndR}{\mathcal{I}_r} % Ensemble des probabilites independantes sur Z + restrictions
%% espaces de probabilites
\def\Prob{\mathbb{P}} % probabilite sur l'espace de la chaine
\def\Exp{\mathbb{E}} % esperance sur l'espace de la chaine
\def\BarExp{\bar{\mathbb{E}}} % esperance sur l'espace  de l'algo
\def\pbar{\bar{\mathbb{P}}} % probabilite sur l'espace de l'algo
%% variables al�atoires et realisations
\newcommand{\tv}{\ensuremath{\mathbf{t}}} % Vecteur des var cachees.(obs)
\newcommand{\sv}{\ensuremath{\mathbf{s}}} % Vecteur des var cachees.(obs)
\newcommand{\Tv}{\ensuremath{\mathbf{T}}} % Vecteur des var cachees.(obs)
\newcommand{\Sv}{\ensuremath{\mathbf{S}}} % Vecteur des var cachees.(obs)
\newcommand{\Wv}{\ensuremath{\mathbf{W}}} % Vecteur des var observees.(obs)
\newcommand{\wv}{\ensuremath{\mathbf{w}}} % Vecteur des var observees.(obs)
\newcommand{\Xv}{\ensuremath{\mathbf{X}}} % Vecteur des var observees.(obs)
\newcommand{\xv}{\ensuremath{\mathbf{x}}} % Vecteur des var observees.(obs)
\newcommand{\Yv}{\ensuremath{\mathbf{Y}}} % Vecteur des var observees.(obs)
\newcommand{\Zv}{\ensuremath{\mathbf{Z}}} % Vecteur des var cachees.(obs)
\newcommand{\yv}{\ensuremath{\mathbf{y}}} % Vecteur des var observees.(obs)
\newcommand{\zv}{\ensuremath{\mathbf{z}}} % Vecteur des var cachees.(obs)
\newcommand{\Ze}{\mathcal{Z}} % Espace d'etat du processus cach\'e.
\newcommand{\B}{{\cal B}}
\newcommand{\taubig}{{\cal T}}
\newcommand{\Be}{\underline{{\cal B}}}
\newcommand{\Phie}{\underline{\Phi}}
\newcommand{\zero}{\ensuremath{\mathbf{0}}}
\def\t{\theta} %parametre
%% Symboles generaux
\def\NNset{\mathbb{N}} % entiers  naturels
\def\Nset{\mathbb{Z}_+} % entiers  naturels
\def\Rset{\mathbb{R}} % reels
%\def\zero{{\mbox{\rm 0\hspace{-0.35em}0}}}  %
\def\un{{\mbox{\rm 1\hspace{-0.25em}I}}}  % indicatrice
\def\ie{\textit{i.e.} } % id est
\def\wp1{\mathrm{w.p.} 1}  % with respect to
\newcommand{\etal}{{\em et al.}} % et al.
%%  GESTION DES DIALOGUES entre AUTEURS
\newenvironment{commentG}
 {\begin{quote}\color{green}\begin{sffamily}}
 {\end{sffamily}\color{black}\end{quote}}
%

\usepackage{graphicx,multirow}				% Use pdf, png, jpg, or epsÂ§ with pdflatex; use eps in DVI mode
\usepackage[page]{appendix}								% TeX will automatically convert eps --> pdf in pdflatex		
\usepackage{amssymb,amsmath,amsfonts,amssymb,hyperref}

\usepackage[svgnames]{xcolor}
\hypersetup{
    colorlinks,
    citecolor=SeaGreen,
    filecolor=black,
    linkcolor=Indigo,
    urlcolor=black
}

\usepackage{dsfont}
\usepackage{natbib}

%\usepackage{algorithm}

\usepackage{algorithm2e}
\RestyleAlgo{ruled}
%
%%\usepackage{subcaption}
%\usepackage{algorithmic} %<-- !
%\usepackage[most]{tcolorbox}
%\usepackage{algpseudocode}

\usepackage[position=bottom]{subfig}
\usepackage{url}
\usepackage[table]{xcolor}
\makeatletter
\g@addto@macro{\UrlBreaks}{\UrlOrds}
\makeatother

\newcommand{\Pedro}[1]{\textcolor{blue}{[#1]}}
\newcommand{\JA}[1]{\textcolor{red}{[#1]}}
